Locally Optimal Eigenvectors of Regular Simplex Tensors

Identifying locally optimal solutions is an important issue given an optimization model. In this paper, we focus on a special class of symmetric tensors termed regular simplex tensors, which is a newly-emerging concept, and investigate its local optimality of the related constrained nonconvex optimization model. This is proceeded by checking the first-order and second-order necessary condition sequentially. Some interesting directions concerning the regular simplex tensors, including the robust eigenpairs checking and other potential issues, are discussed in the end for future work.

==> Diri.tex <==
\section{Relation to  the data  with  the  Dirichlet  distribution}\label{dirisec}

In  this  part,  we will  further   investigate  the  skewness  distribution    for the data  with  the  Dirichlet  distribution,  whose  definition  is   given  as   follows:  
\begin{definition}[\textbf{The Dirichlet  distribution}]\cite{2006Pattern}\label{defi_diri}
	The Dirichlet  distribution  is a multivariate one over 
	$K$ random variables                 $  y_{k}$,  % $ 0 \le   y_{k} \le  1$  
	where 
	$ k$ $ =$  1,2, $\dots $,  $K$, 
	subject to the constraints
	$
	0 \le  y_{k} \le  1, 
	\sum_{k=1}^{K}
	y_{k}
	=1$.
	% \begin{align}
	% 0 \le  y_{k} \le  1, 
	% \nonumber  \\
	% \sum\limits_{k=1}^{K}
	% y_{k}
	% =1
	% \end{align}
	Denote 
	$  \mathbf y =(y_{1},y_{2},\dots,y_{K})^{\mathrm T} $,
	and
	$  \boldsymbol {\alpha} =(\alpha_{1},\alpha_{2},\dots,\alpha_{K})^{\mathrm T} $, where $ \alpha_{i}  > 0$  for  each $i$,  it  follows:
	\begin{align}\label{diri_define}
	Dir(\mathbf y|\boldsymbol {\alpha})
	=
	\frac
	{ \Gamma(\alpha_{0})}
	{ \Gamma(\alpha_{1}) \Gamma(\alpha_{2}) \dots \Gamma(\alpha_{K})}
	\prod\limits_{k=1}^{K}
	y_{k}^{  \alpha_{k}-1  } ,
	\end{align}
	where
	$
	\Gamma(\alpha)
	=
	\int_{0}^{+\infty}
	t^{ \alpha-1}
	e^{-t}
	d t
	$
	is the   Gamma  function, and 
	$
	\alpha_{0}= \sum_{k=1}^{K}
	\alpha_{k}.
	$
	$ \boldsymbol {\alpha}$ is called the  concentration parameter, which controls  sparsity or concentration degree.
	Note  that  due  to the  sum-to-one  constraint, the free  degree of the data  that  follows  Dirichlet  distribution  with  $n$  variables  is  $n-1$. 
	% From the perspective of  geometry, the $n$-dimensional support set of Dirichlet distribution is an  $n-1$  dimensional  simplex.   Note that  when    $  \alpha_{1} =\alpha_{2}= \dots =\alpha_{K}$ =1,  the samples are uniformly distributed in the simplex.
\end{definition}


After  some  theoretical  derivations,  another  interesting  finding   was   revealed  concerning   the   skewness   relationship   between  the  simplex   and  the data  with  the  Dirichlet  distribution,   and  the  details  are as    follows. 

\subsection{Cases  without   noise}
Denote the data   $ \mathbf X$   that  follows  the Dirichlet  distribution  as
\begin{align}\label{datadiri}
\mathbf X=[ \mathbf y_{1},  \mathbf y_{2},  \dots, \mathbf y_{P} ]  
=
\begin{bmatrix}
\mathbf x_{1}^{\mathrm T}  
\\
\mathbf x_{2}^{\mathrm T}
\\
\vdots
\\
\mathbf x_{n}^{\mathrm T} 
\end{bmatrix}
\in   \mathbb  R^{n \times P} ,
\end{align}
where  $ \mathbf y_{i}$ $ (i=1,2, \dots, P)  \in   \mathbb  R^{n \times 1} $  satisfies  (\ref{diri_define}), and $ P$ is  the number  of sample  points,
and  $ \mathbf x_{i}$ $ (i=1,2, \dots, n)  \in   \mathbb  R^{1 \times P} $. 
In  addition,   the concentration parameter   is  always  set  to   $  \alpha_{1} =\alpha_{2}= \dots =\alpha_{K} = \alpha$, i,e,.   $   \boldsymbol {\alpha} = \alpha \mathbf  1_{n}$, where $ \alpha >0$. 
We  have  the  following  theorem:

\begin{theorem}\label{Theorem_dirchlet}
	For  the data  that  satisfies  the Dirichlet   distribution with  $n$ random variables, as shown in (\ref{datadiri}) with $   \boldsymbol {\alpha} = \alpha \mathbf  1_{n}$,  the  skewness  distribution  is  proportional  to that of the simplex with   $n$ vertices.  
\end{theorem}
 


\begin{proof}
 For the data that  satisfies the Dirichlet  distribution as  in (\ref{datadiri}),  it  holds  that 
\begin{align}\label{6euqal} 
\centering
\nonumber
&  {\rm  E}
\{
\mathbf x_{\it i}
\}
=
\frac
{\alpha_{\it i}	}
{\alpha_{ 0}	} , 
{\rm  E}
\{
\mathbf x_{\it i}^{2}
\}
=
\frac
{(\alpha_{\it i}+1)\alpha_{\it i}	}
{(\alpha_{ 0}+1)\alpha_{ 0}	} , 
\\  \nonumber  
&{\rm  E}
\{
\mathbf   x_{\it  i} 
\mathbf   x_{\it j}
\}
=
\frac
{\alpha_{\it i}\alpha_{\it j}	}
{(\alpha_{ 0}+1)\alpha_{ 0}	}
,
{\rm  E}
\{
\mathbf  x_{\it i}^{3}
\}
=
\frac
{    (\alpha_{\it i}+2)(\alpha_{\it i}+1)\alpha_{\it i}	}
{   M	}  , 
\\    
& \rm  {E}
\{
\mathbf  x_{\it i}^{2}
\mathbf   x_{\it j}
\}
=
\frac
{(\alpha_{\it i}+1)\alpha_{\it i}	\alpha_{\it j}		}
{\it  M		}
,
{\rm  E}
\{
\mathbf  x_{\it i}
\mathbf   x_{\it j}
\mathbf   x_{\it k}
\}
=
\frac
{\alpha_{\it i}\alpha_{\it j}	\alpha_{\it k}		}
{\it  M	}, 
\end{align} 
where   $M=(\alpha_{ 0}+2)(\alpha_{ 0}+1)\alpha_{ 0}$   for  simplicity.
%\begin{equation} \label{u_constraint}
%\begin{cases}
%\sum\limits_{i=1}^{n}
%  u_{i}
%  = 
%u_{1} +  u_{2} + \dots  u_{n}  =0 
% \\
%\sum\limits_{i=1}^{n}
% u_{i}^{2}  
% =
%u_{1}^{2} +  u_{2}^{2} + \dots  u_{n}^{2}  =1 
%\end{cases}.
%\end{equation}
Denote  
 \begin{align}
 \notag
 \mathbf z =   \mathbf u^{\mathrm  T}\mathbf X  = \sum_{\it  i=\rm 1}^{\it  n} u_{\it  i}\mathbf x_{\it  i}= u_{1}\mathbf x_{1} +u_{2}\mathbf x_{2} + \dots + u_{n}\mathbf x_{n}
\in  \mathbb  R^{1  \times P},
\end{align}
 we  analyze  its    skewness by   separately    calculating the numerator and demonator. 
First,  since    $   \boldsymbol {\alpha} = \alpha \mathbf  1_{n}$,   it can be derived that   
%\begin{align}\label{}
%skew(\mathbf u^{\mathrm  T}\mathbf R)
%&= 
%skew( u_{1}\mathbf x_{1} +u_{2}\mathbf x_{2} + u_{n}\mathbf x_{n} )
%\\  \nonumber 
%&=
%skew(  )
%=
%\frac
%{
%	k_{3} (\mathbf z)
%}
%{
%	(  k_{2} (\mathbf z) )
%	^{\frac 3 2}
%}
%\end{align}
\begin{align}\label{}
{\rm E}(\mathbf z)
%=
%{\rm E} (\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}\mathbf x_{\it  i}  )	
=
\sum\limits_{i=1}^{n}  u_{i}   {\rm E}  (\mathbf x_{\it i})	
=
\sum\limits_{i=1}^{n}  u_{i}  \frac
{\alpha_{ i}	}
{\alpha_{ 0}	}	
=
\frac
{\alpha	}
{\alpha_{ 0}	}	\sum\limits_{i=1}^{n}  u_{i}
=0	.
\end{align}


Therefore,  we  have  that  for   $	k_{3} (\mathbf z)$, it  holds  that 
\begin{align}\label{k3zori}
&	k_{3} (\mathbf z)
=
{\rm  E}
\{
(
\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}\mathbf x_{\it  i}  - 0 )
^{3} 
\}
\nonumber    \\
& = 
{\rm E}
\{
\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 3}\mathbf x_{\it  i}^{\rm 3}
 +
3\sum\limits_{1 \le \it  i < \it  j \le n}^{\it  n} 
(u_{\it  i}^{\rm 2}u_{\it  j}  \mathbf x_{\it  i}\mathbf x_{\it  j}^{\rm 2}
+
u_{\it  i} u_{\it  j}^{\rm 2}     \mathbf x_{\it  i}^{\rm 2}\mathbf x_{\it  j}
)
\nonumber   \\
&
+
6\sum\limits_{1 \le \it  i < \it  j < \it k \le n}^{\it  n} 
u_{\it  i} u_{\it  j}  u_{\it  k}
\mathbf x_{\it  i} \mathbf x_{\it  j} \mathbf x_{\it  k}
\}	.
\end{align}

%Substituting  the terms  in  (\ref{6euqal})  into   (\ref{k3zori})  yields
%\begin{align}\label{k3z_simple1}
%k_{3} (\mathbf z)
%= 
%\frac 
%{6}
%{M}
%&(
%\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 3}
%+
%\sum\limits_{1 \le  \it  i < \it  j\le n}^{\it  n} 
%(u_{\it  i}^{\rm 2}u_{\it  j}
%+ 
%u_{\it  i} u_{\it  j}^{\rm 2}
%)
%%\nonumber   \\
%%& 
%+
%\sum\limits_{1 \le \it  i < \it  j < \it k \le n}^{\it  n} 
%u_{\it  i} u_{\it  j}  u_{\it  k}
%).  
%%\nonumber   \\
%%& 
%%= 
%%\frac 
%%{6}
%%{M}   ( a+b+c  ) 	
%\end{align}

By  utilizing  the  two  constraints, i.e.,   $ \mathbf   u^{\mathrm T}   \mathbf   u =1,  
\mathbf   u^{\mathrm T}   \mathbf   1_{n} =0$,  we  have  that 
\begin{align}\label{sum_u3}
0
=
(\sum\limits_{i=1}^{n}
u_{i})^{3}
&= 
\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 3}
+
3 \sum\limits_{1 \le  \it  i < \it  j\le n}^{\it  n} 
(u_{\it  i}^{\rm 2}u_{\it  j}
+ 
u_{\it  i} u_{\it  j}^{\rm 2}
)
\nonumber   \\
& +
6 \sum\limits_{1 \le \it  i < \it  j < \it k \le n}^{\it  n} 
u_{\it  i} u_{\it  j}  u_{\it  k}, 	
\end{align}
and
\begin{align}\label{u1_multi_u2}
0
=
(\sum\limits_{i=1}^{n}
u_{i})(\sum\limits_{i=1}^{n}
u_{i}^{2})
= 
\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 3}
+
\sum\limits_{1 \le  \it  i < \it  j\le n}^{\it  n} 
(u_{\it  i}^{\rm 2}u_{\it  j}
+ 
u_{\it  i} u_{\it  j}^{\rm 2}
)	.
\end{align}


Based  on   (\ref{sum_u3})   and  (\ref{u1_multi_u2}), we   derive that 
\begin{equation}\label{two_terms}
\begin{cases}
\sum\limits_{1 \le  \it  i < \it  j\le n}^{\it  n} 
(u_{\it  i}^{\rm 2}u_{\it  j}
+ 
u_{\it  i} u_{\it  j}^{\rm 2}
)	
=- \sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 3} 
\\
\sum\limits_{1 \le \it  i < \it  j < \it k \le n}^{\it  n} 
u_{\it  i} u_{\it  j}  u_{\it  k}
=
\frac 13 \sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 3}
\end{cases} .
\end{equation}

Then,  substituting    (\ref{two_terms})     into   (\ref{k3zori})  leads  to     

\begin{align}\label{k3zfinal}
k_{3} (\mathbf z)
\varpropto
\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 3}	.  
\end{align}


Similar to the process  for $ k_{3} (\mathbf z)$ as  analyzed above, we can   simplify  $ k_{2} (\mathbf z)$, which  follows:
\begin{align}\label{k2zori}
k_{2} (\mathbf z)
&=
{\rm  E}
\{
(
\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}\mathbf x_{\it  i}   )
^{2} 
\}
%\nonumber    \\
%&
= 
{\rm E}
\{
\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 2}\mathbf x_{\it  i}^{\rm 2}
+
2\sum\limits_{1 \le \it  i < \it  j \le n}^{\it  n} 
u_{\it  i}  u_{\it  j}  \mathbf x_{\it  i}\mathbf x_{\it  j}
\}  .
%\nonumber    \\
%&= 
%\frac
%{2}
%{  (\alpha_{ 0}+1)\alpha_{ 0}  }
%\{
%\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 2} 
%+
%\sum\limits_{1 \le \it  i < \it  j \le n}^{\it  n} 
%u_{\it  i}  u_{\it  j} 
%\}	.   
\end{align} 


It holds  that 
\begin{align}\label{}
0
&=
(\sum\limits_{i=1}^{n}
u_{i})^{2}
= 
\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 2}
+
2 \sum\limits_{1 \le  \it  i < \it  j\le n}^{\it  n} 
u_{\it  i}^{\rm 2}u_{\it  j}, 
\end{align}
which  indicates  that 
\begin{align}\label{simresult} 
 \sum\limits_{1 \le  \it  i < \it  j\le n}^{\it  n} 
u_{\it  i}^{\rm 2}u_{\it  j}  =   - \frac  1 2  \sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 2}.
\end{align}
Substitute   (\ref{simresult})   into   (\ref{k2zori}),   we  have 
\begin{align}\label{k2zfinal}
k_{2} (\mathbf z)
= 
\frac
{(\alpha_{\it i}+1)\alpha_{\it i}  - \alpha_{\it i} \alpha_{\it j} 	}
{(\alpha_{ 0}+1)\alpha_{ 0}	}
= 
\frac
{\alpha	}
{(\alpha_{ 0}+1)\alpha_{ 0}	},
\end{align}
where $ \alpha_{\it i} =\alpha_{\it j}= \alpha$.  
By combining (\ref{k3zfinal})   with  (\ref{k2zfinal}), we  deduce that 
\begin{align}\label{}
skew(\mathbf u^{\mathrm  T}\mathbf X)
\varpropto
\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 3},
\end{align}
which is  proportional   to the  skewness   of the simplex with   $n$ vertices, as  shown in (\ref{skewui3}).
$\blacksquare$
\end{proof}







%  The    proof  is  given   in  \ref{proof_dirchlet}. 
Note  that  such  a   conclusion   motivates  us  to  consider  the  application  of  the new  property  in  the  field  of  hyperspectral   unmixing,   whose  detailed   descriptions  and  experimental results  using  simulation  and  real  data  set     are  presented  in  the   section V.  


\subsection{Cases  with  Gaussian  noise} 
In this part,
we  further  consider    the  Dirichlet   distribution  data,  which is  corrupted by  the Gaussian  white  noise. 
Denote   
$\mathbf N  \in   \mathbb  R^{n \times P} $  is  the  Gaussian  white  noisy    data,  which is  independent  to $\mathbf X$, and takes the same form as (\ref{datadiri}). 
For  the  row of $\mathbf N $  denoted    $\mathbf n_{i} $, it    satisfies 
$ {\rm E}(\mathbf n_{i}) =0,  k_{2}( \mathbf n_{i}) = \sigma^{2}$  for  all   $i=1,2, \dots, n$.
Then, we have the  following   result:
\begin{theorem}\label{Theorem_dirchletnoie}
	Given   the data  that  satisfies  the Dirichlet   distribution with  $n$ random variables, as shown in (\ref{datadiri}).
	Denote $ \mathbf X_{n}=  \mathbf X +  \mathbf N$. 
	It holds  that    the  skewness   for $ \mathbf X_{n}$   is  also  proportional  to that of the simplex with   $n$ vertices.     
\end{theorem}

 



Before  proving    Theorem  \ref{Theorem_dirchletnoie},  the  following  lemma  is  very   useful\cite{sti}:
\begin{lemma}\label{indpend}
	Let  $ X$ and    $ Y$ be  two  independent  random  variables, and  let  
	$g(X)$  be  a  function   only  of $ X $ and  
	$h(Y)$  be  a  function   only  of $ Y$ .
	Then, 
	it  holds
	\begin{align}\label{independentE}
	\rm  {E}  ( \it g( X) h(  Y))=
	\rm  {E}  ( \it g( X)) 
	\rm  {E}	 (\it   h( Y)).
	\end{align}
\end{lemma}


%\section{Experimental  Results   }


Then  we  proceed  our   proof  for   Theorem  \ref{Theorem_dirchletnoie}.


\begin{proof}
For the  skewness  of  $\mathbf X_{n}$   projected  along  the direction $ \mathbf u$, it holds that 
$skew(  \mathbf u^{\mathrm  T} \mathbf X_{n}   )
=
skew(  \mathbf u^{\mathrm  T} ( \mathbf X +  \mathbf N)  ) 
=
skew(  \mathbf u^{\mathrm  T}   \mathbf X +  \mathbf u^{\mathrm  T} \mathbf N  ) 
$.
Correspondingly, we     calculate the numerator and denominator, which  follows:   
\begin{align}\label{k3znoise}
k_{3}  ( &  \mathbf u^{\mathrm  T}   \mathbf X  +  \mathbf u^{\mathrm  T} \mathbf N ) 
\nonumber  \\
& =
\rm  {E}
 \{
(  \mathbf u^{\mathrm  T}   \mathbf X +  \mathbf u^{\mathrm  T} \mathbf N  )^{3}
\}  
\nonumber  \\
&
=
\rm  {E}
\{
(  \mathbf u^{\mathrm  T}   \mathbf X  )^{3}
\}
+
3
\rm  {E}
\{
( \mathbf u^{\mathrm  T}   \mathbf X )^{2}   \mathbf u^{\mathrm  T} \mathbf N	
\}
\nonumber \\
& \quad  +
3
\rm  {E}
\{
\mathbf u^{\mathrm  T}   \mathbf X 
(   \mathbf u^{\mathrm  T} \mathbf N )^{2}	
\}
+
\rm  {E}
\{
(   \mathbf u^{\mathrm  T} \mathbf N )^{3}	
\}
\nonumber \\
& =
\rm  {E}
\{
(  \mathbf u^{\mathrm  T}   \mathbf X  )^{3}
\}
+
3
\rm  {E}
\{
( \mathbf u^{\mathrm  T}   \mathbf X )^{2}
\}
\rm  {E}
\{   \mathbf u^{\mathrm  T} \mathbf N	
\}
\nonumber \\
& \quad  +
3
\rm  {E}
\{
\mathbf u^{\mathrm  T}   \mathbf X 
\}
\rm  {E}
\{
(   \mathbf u^{\mathrm  T} \mathbf N )^{2}	
\} 
+
\rm  {E}
\{
(   \mathbf u^{\mathrm  T} \mathbf N )^{3}	
\}
\nonumber  \\
&
=
\rm  {E}
\{
(  \mathbf u^{\mathrm  T} \mathbf X  )^{3}
\}
=
\it k_{ \rm 3} (\mathbf z)
\varpropto
\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 3}.
\end{align}
where  in the  third equation,  we utilize  (\ref{independentE}), and  in the  fourth one, we use the  fact  that 
$\rm  {E}
\{   \mathbf u^{\mathrm  T} \mathbf N	
\}
=  \rm  {E}
\{   \mathbf u^{\mathrm  T} \mathbf X	
\}
=0
$, and the   higher-order  statistics   for  
 the  noisy  data $\mathbf N$ that 
follows  Gaussian  distribution   along  any  direction 
are   always  equal to zero.

Similarly,  it  holds that 
\begin{align}\label{k2znoise}
&  k_{2}  ( \mathbf u^{\mathrm  T}   \mathbf X +  \mathbf u^{\mathrm  T} \mathbf N ) 
\nonumber  \\
& =
\rm  {E}
\{
(  \mathbf u^{\mathrm  T}   \mathbf X +  \mathbf u^{\mathrm  T} \mathbf N  )^{2}
\}  
\nonumber  \\
&
=
\rm  {E}
\{
(  \mathbf u^{\mathrm  T}   \mathbf X  )^{2}
\}
+
2
\rm  {E}
\{
 \mathbf u^{\mathrm  T}   \mathbf X
\}
\rm  {E}
\{   \mathbf u^{\mathrm  T} \mathbf N	
\} 
+
\rm  {E}
\{
(   \mathbf u^{\mathrm  T} \mathbf N )^{2}	
\}
\nonumber  \\
&
=
\it k_{\rm  2} (\mathbf z)
+ 
\rm  {E}
\{
(   \mathbf u^{\mathrm  T} \mathbf N )^{2}	
\} 
\nonumber  \\
&
=\frac
{\alpha	}
{(\alpha_{ 0}+1)\alpha_{ 0}	} +\sigma^{2},
\end{align}
which  is   a  constant  irrelevant  to  $ \mathbf u$.
Combining   (\ref{k3znoise}) with  (\ref{k2znoise})  yields 
\begin{align}
skew(  \mathbf u^{\mathrm  T} \mathbf X_{n}   )
\varpropto
\sum\limits_{\it  i=\rm 1}^{\it  n} u_{\it  i}^{\rm 3},
\end{align}
and  the proof  is complete.
$\blacksquare$
\end{proof}


This  indicates  that   the    skewness  distribution  of  the data  with  the Dirichlet   distribution  is  robust  to   the  Guassian  noise,  and  this  also   due  to  the  fact  that  the   third-oder  statistic   of  the  Gaussian   distribution  will  be  zero, as  analyzed  in  (\ref{k3znoise}).

\begin{lemma}\label{weyltheo}
Assume  that 
$\mathbf A$, $\mathbf B$ is Hermitian  matrix,  and  the  eigenvalues are  sorted  in  a  ascending  order. 
\begin{equation}
\begin{aligned}
\lambda_{1}(\boldsymbol{A}) & \leqslant \lambda_{2}(\boldsymbol{A}) \leqslant \cdots \leqslant \lambda_{n}(\boldsymbol{A}) \\
\lambda_{1}(\boldsymbol{B}) & \leqslant \lambda_{2}(\boldsymbol{B}) \leqslant \cdots \leqslant \lambda_{n}(\boldsymbol{B}) \\
\lambda_{1}(\boldsymbol{A}+\boldsymbol{B}) & \leqslant \lambda_{2}(\boldsymbol{A}+\boldsymbol{B}) \leqslant \cdots \leqslant \lambda_{n}(\boldsymbol{A}+\boldsymbol{B})
\end{aligned}
\end{equation}

\begin{equation}
\lambda_{i}(\boldsymbol{A}+\boldsymbol{B}) \geqslant\left\{\begin{array}{c}
\lambda_{i}(\boldsymbol{A})+\lambda_{1}(\boldsymbol{B}) \\
\lambda_{i-1}(\boldsymbol{A})+\lambda_{2}(\boldsymbol{B}) \\
\vdots \\
\lambda_{1}(\boldsymbol{A})+\lambda_{i}(\boldsymbol{B})
\end{array}\right.
\end{equation}
\begin{equation}
\lambda_{i}(A+B) \leqslant\left\{\begin{array}{c}
\lambda_{i}(\boldsymbol{A})+\lambda_{n}(B) \\
\lambda_{i+1}(\boldsymbol{A})+\lambda_{n-1}(\boldsymbol{B}) \\
\vdots \\
\lambda_{n}(\boldsymbol{A})+\lambda_{i}(\boldsymbol{B})
\end{array}\right.
\end{equation}
for  $i=1,2,\dots, n$.
\end{lemma}

==> ES.tex <==
\section{Skewness  for the regular polygon}\label{polygon}

The  presented  Theorem \ref{Theorem_optimal}  has revealed  the one-to-one  corresponding  relationship between the locally  skewness  directions  and  altitudes of the simplex. 
In  this part, we  further  provide  an  auxiliary  lemma to  illustrate  the  special characteristics  of  the simplex  and  the  triangle. 
 

\begin{lemma}\label{Theorem_ploygon}
	For  the  regular  polygon  with  $p$  vertices  where  $p$ $\ge$ 4,  its  skewness  value   projected  along any  direction  will  always be  equal to  0.  
\end{lemma}


Before  proceeding  our  proof,  the  following  theorem is  very  useful:
\setcounter{theorem}{3}
\begin{theorem}(Ref \cite{upperbound})\label{upperbound}
	The number of  real  Z-eigenpairs for  symmetric tensor  of order $m$ and dimension $ n $ is  at most
	\begin{equation}\label{at_most}
	M(m,n)=
	\frac {(m-1)^{n}-1}  {m-2}.
	\end{equation}
\end{theorem}









Note  that   for  different  data $ \mathbf R$ and  thus  different   symmetric  tensors, 
the number of  these   locally  optimal  solutions (denoted $K$)   may    vary.  Theorem  \ref{upperbound}  provides  a  upper  bound   for  the  number  of  eigenpirs of  tensor, 
and thus also  a  weak   upper  bound  for  $K$.
 For  example,   for  the   symmetric tensors  of order 3 and dimension 3, it  also  always  holds   that 
$M$(3,3) = 7 and $ K$ $\le$ 7.
Equipped  with  such  a  theory, we  begin to proceed  our  proof for  the presented   Lemma \ref{Theorem_ploygon}.
\begin{proof}
	The proof   mainly   includes   two  steps: 
	
	\textbf{Step 1:}  	we    show  that  the skewness value of the   regular  polygon  with  $p$  vertices 
	($p$ $\ge$ 4)  along  any  direction  is  a  constant;
	
	\textbf{Step 2:}   we   demonstrate that  this  constant  is  equal to 0. 
	
	Step  1  is  proved  by contradiction.   
	On  the  one  hand, assume  that   for  the   regular  polygon  with  $p$  vertices 
	($p$ $\ge$ 4)  in  a  2D  plane,  there  is  at  least  one  locally  optimal   direction (denoted $\mathbf u_{1}$),  
	according  to  the  symmetry  property  of  the  regular  polygon, 
	then  the  direction  which    rotates   $\mathbf u_{1}$  with  an  angle  of  $ \frac  {2\pi i} {p}$  ($i=1, 2 , \dots, p$)     will  also be  one locally  optimal   direction.
	Thus,   we  can  conclude  that  $ K \ge p \ge  4$. 
	On the other  hand,  the  third-order  statistical  tensor  of  the   regular  polygon   in  a  2D  plane
	is  always with   a   size  of   2  $\times$ 2  $\times$ 2,  and it  should  hold  that  $ K \le  M(2,3) = 3$    based  on  Theorem  \ref{upperbound}. 
	Therefore,  there  exists  contradiction  and the  assumption do  not  hold,  and  we  can conclude that  the  number of  locally  optimal   directions  is  equal to  0,  which  implies  that  the claim  in  step  1  is  true.  
	
	Then,  for  step 2,   it is  enough    to    show  that  the  skewness  value  in  one  certain  direction  for the   regular  polygon with $p$ $\ge $ 4  is  equal to  0. 
	First,  the  $p$  vertices  for  the  regular  polygon   can   be  denoted  as  matrix  with  the  following  form:
\begin{align}
\notag
\mathbf {R}
= 
\begin{bmatrix}
   sin(0)   &     sin(\frac  {2\pi } {p})  &   sin(\frac  {4\pi } {p})  & \dots   &  sin(\frac  {2\pi (p-1)} {p}) \\  
 cos(0)   &     cos(\frac  {2\pi } {p})  &  cos(\frac  {4\pi } {p})  &  \dots   &  cos(\frac  {2\pi (n-1)} {p})
\end{bmatrix} . 
\end{align}
It  is  easily  checked  that  each  row  of  $ \mathbf {R}$  is  with  zero  mean,   due  to  the  fact  
that  $sin(\frac  {2\pi i } {p}) (i=0,1,2,\dots, p-1)$  is a  periodical  function  whose  period is  $p$.
Next,  we   consider  the  skewness  value  of  $ \mathbf {R}$ along  the    horizontal  direction $ \mathbf  w =[1 ,  0]^{\mathrm T}$,   and  we  only need  to  calculate  the  numerator, which  follows:
\begin{align}
k_{3} (\mathbf  w^{\mathrm T}\mathbf {R})
\notag
&=
\sum\limits_{i=0}^{p-1}  sin^{3}(\frac  {2\pi i } {p})
=
 \sum\limits_{i=0}^{p-1}  sin(\frac  {2\pi i } {p}) (1-cos^{2}(\frac  {2\pi i } {p})) 
\\  \nonumber 
& =
 \sum\limits_{i=0}^{p-1}  sin(\frac  {2\pi i } {p}) -  \sum\limits_{i=0}^{p-1}  sin(\frac  {2\pi i } {p}) cos^{2}(\frac  {2\pi i } {p})
 =
 0. 
\end{align}
And  the  proof  is  complete. $\blacksquare$ 
\end{proof}


==> deshared.tex <==

% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{amsmath}
\usepackage{geometry}
\usepackage{amssymb}
\usepackage{caption,subcaption}
\usepackage{multirow}
\usepackage{makecell} 
\usepackage{threeparttable}


\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
%\newsiamremark{corollary}{Corollary}
%\newtheorem{theorem}{\textbf{Theorem}}
%\newtheorem{lemma}{\textbf{Lemma}}
%\newtheorem{proof}{Proof}[section]
%\newtheorem{definition}{\textbf{Definition} }
%\newtheorem{remark}{\textbf{Remark}}
\newtheorem{conjecture}{\textbf{Conjecture}}
\newtheorem{property}{\textbf{Property}}
\newtheorem{comment}{\textbf{Comment}}


% Sets running headers as well as PDF title and authors
\headers
{
%	Robust  Eigenvectors of  regular  simplex tensors
Locally  Optimal   Eigenvectors of  Regular  Simplex Tensors
}
{ 
	Lei Wang
}

%\headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}
% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.

\title{
%	Robust  Eigenvectors of  regular  simplex tensors
Locally  Optimal   Eigenvectors of  Regular  Simplex Tensors
	\thanks
	{Submitted to the editors DATE.
\funding{
	%This research did not receive any special   grant from funding agencies in the public, commercial, or not-for-profit sectors.
	This work was partially supported by National Natural Science Fund of China (62271090), Chongqing Natural Science Fund (cstc2021jcyj-jqX0023), National Key R\&D Program of China (2021YFB3100800), CCF Hikvision Open Fund (CCF-HIKVISION OF 20210002), CAAI-Huawei MindSpore Open Fund, and Beijing Academy of Artificial Intelligence (BAAI).
}
}
}


%\author{Lei  Wang
%	\thanks{Aerospace Information Research Institute, Chinese Academy of Sciences, Beijing 100094, China;}
%\and
%		\thanks{
%School  of Electronic, Electrical and Communication Engineering,  the University of the Chinese Academy of Sciences, Beijing 100049;}
%\and
% 	\thanks{Key Laboratory of  Technology in Geo-Spatial Information Processing and Application System, Chinese Academy of Science, Beijing 100190, China. (\email{wanglei179@mails.ucas.ac.cn})} 
%\and Xiurui Geng
%	\thanks{Aerospace Information Research Institute, Chinese Academy of Sciences, Beijing 100094, China;}
%\and
%\thanks{
%	School  of Electronic, Electrical and Communication Engineering,  the University of the Chinese Academy of Sciences, Beijing 100049;}
%\and
%\thanks{Key Laboratory of  Technology in Geo-Spatial Information Processing and Application System, Chinese Academy of Science, Beijing 100190, China.  (\email{gengxr@sina.com.cn}).} 
%}


%\author{ 
%	%Lei Wang, Xiurui Geng, Lei Zhang 
%	\thanks{
%		Lei Wang   are  with  the School of Microelectronics and Communication
%		Engineering, Chongqing University, Chongqing 400044, China; 
%	\quad Xiurui Geng  is  with 	Aerospace Information Research Institute, Chinese Academy of Sciences, Beijing 100094, China;
%School  of Electronic, Electrical and Communication Engineering,  the University of the Chinese Academy of Sciences, Beijing 100049;
%	   Key Laboratory of  Technology in Geo-Spatial Information Processing and Application System, Chinese Academy of Science, Beijing 100190, China. 
%	   % (Corresponding authors: Xiurui Geng, Lei Wang. Email:gengxr@sina.com.cn; wanglei179@mails.ucas.ac.cn.).
%   }}


\author{Lei Wang\thanks{the School of Microelectronics and Communication
		Engineering, Chongqing University, Chongqing 400044, China;
		(\email{wanglei179@mails.ucas.ac.cn;leizhang@cqu.edu.cn}).
	}
			(Corresponding author: Lei Wang. Email:wanglei179@mails.ucas.ac.cn)



\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

